The Brain Tumor Segmentation (BraTS) Challenge 2023: Brain MR Image Synthesis for Tumor Segmentation (BraSyn)

Automated brain tumor segmentation methods have become well-established and reached performance levels offering clear clinical utility. These methods typically rely on four input magnetic resonance imaging (MRI) modalities: T1-weighted images with and without contrast enhancement, T2-weighted images, and FLAIR images. However, some sequences are often missing in clinical practice due to time constraints or image artifacts, such as patient motion. Consequently, the ability to substitute missing modalities and gain segmentation performance is highly desirable and necessary for the broader adoption of these algorithms in the clinical routine. In this work, we present the establishment of the Brain MR Image Synthesis Benchmark (BraSyn) in conjunction with the Medical Image Computing and Computer-Assisted Intervention (MICCAI) 2023. The primary objective of this challenge is to evaluate image synthesis methods that can realistically generate missing MRI modalities when multiple available images are provided. The ultimate aim is to facilitate automated brain tumor segmentation pipelines. The image dataset used in the benchmark is diverse and multi-modal, created through collaboration with various hospitals and research institutions.

==> 3_results.tex <==
\section{Results}

Baseline results can be discussed here

==> 4_discussion.tex <==
\section{Discussion}

Discussion goes here





==> Notes.tex <==
# Important notes/TO-DO for manuscript goes here 

Please make sure you add the following authors in the next revision of each challenge manuscript.
Verena Chung, Sage Bionetworks
Maria Diaz, Sage Bionetworks
Byrone Cole, Sage Bionetworks
James Eddy, Sage BIonetworks
Jake Albrecht, Sage Bionetworks

It would also be nice to have a consistent description of the Synapse platform: 

Synapse is a collaborative research platform that helps teams share, organize, and discuss their scientific research.  Synapse supports the capacity to create and manage community data challenges, using containerized models for secure evaluation of participant submitted methods.

 
